Context Unlocks Emotions: Text-based Emotion Classification Dataset Auditing with Large Language Models

The lack of contextual information in text data can make the annotation process of text-based emotion classification datasets challenging. As a result, such datasets often contain labels that fail to consider all the relevant emotions in the vocabulary. This misalignment between text inputs and labels can degrade the performance of machine learning models trained on top of them. As re-annotating entire datasets is a costly and time-consuming task that cannot be done at scale, we propose to use the expressive capabilities of large language models to synthesize additional context for input text to increase its alignment with the annotated emotional labels. In this work, we propose a formal definition of textual context to motivate a prompting strategy to enhance such contextual information. We provide both human and empirical evaluation to demonstrate the efficacy of the enhanced context. Our method improves alignment between inputs and their human-annotated labels from both an empirical and human-evaluated standpoint.

==> Tables/mapping_table.tex <==
\begin{table}[]
\caption{Mapping of GoEmotion labels to target datasets}
\label{tab:mapping_emotions}
\centering
\small
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c}{\textbf{Original}} & \textbf{Mapped}      & \multicolumn{1}{c}{\textbf{Original}} & \textbf{Mapped} \\ \midrule
\multicolumn{2}{c}{\textbf{ISEAR}}                           & \multicolumn{2}{c}{\textbf{Daily Dialog}}               \\ \midrule
\multicolumn{1}{c}{Joy}               & Joy                  & \multicolumn{1}{c}{Neutral}           & Neutral         \\ 
\multicolumn{1}{c}{Fear}              & Fear                 & \multicolumn{1}{c}{Anger}             & Anger           \\ 
\multicolumn{1}{c}{Anger}             & Anger                & \multicolumn{1}{c}{Disgust}           & Disgust         \\ 
\multicolumn{1}{c}{Sadness}           & Sadness       & \multicolumn{1}{c}{Fear}              & Fear            \\ 
\multicolumn{1}{c}{Disgust}           & Disgust              & \multicolumn{1}{c}{Happiness}         & Joy             \\ 
\multicolumn{1}{c}{Shame}             & Embarrassment        & \multicolumn{1}{c}{Sadness}           & Sadness  \\ 
\multicolumn{1}{c}{Guilt}             & Remorse              & \multicolumn{1}{c}{Surprise}          & Surprise        \\ \midrule
\multicolumn{2}{c}{\textbf{SemEval 2019 Task 3}}            & \multicolumn{2}{c}{\textbf{Tweet Eval}}       \\ \midrule
\multicolumn{1}{c}{Others}            & All the other labels & \multicolumn{1}{c}{Anger}             & Anger           \\ 
\multicolumn{1}{c}{Happy}             & Joy                  & \multicolumn{1}{c}{Joy}               & Joy             \\ 
\multicolumn{1}{c}{Sad}               & Sadness       & \multicolumn{1}{c}{Optimism}          & Optimism        \\ 
\multicolumn{1}{c}{Angry}             & Anger                & \multicolumn{1}{c}{Sadness}           & Sadness  \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/p_value_table.tex <==
\begin{table*}[]
\caption{p-value test results}
\label{tab:p-value-results}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Test Name                 & Effect Size & Alpha & Power & n   & No. of Groups & Score    \\ \hline
Wilcoxon-Signed-Rank & 0.2         & 0.05  & 0.95  & 47  & -             & 4.76E-05 \\ \hline
Kruskal Wallis          & 0.25        & 0.05  & 0.95  & 486 & 18            & 4.28E-18 \\ \hline
\end{tabular}
\end{table*}

==> Tables/results_bert_emo.tex <==
\begin{table*}[]
\caption{Zero Shot Emotion Recognition Results for Target Datasets}
\label{tab:master_results}
\centering
\begin{tabular}{|c|c|ccc|cc|ccc|}
\hline
                                 & \textbf{ISEAR}  & \multicolumn{3}{c|}{\textbf{Daily Dialog}}                                                        & \multicolumn{2}{c|}{\textbf{Sem Eval 2019 Task 3}}     & \multicolumn{3}{c|}{\textbf{Sem Eval 2018 Task 1}}                                                \\ \hline
                                 & \textbf{Total}  & \multicolumn{1}{c|}{\textbf{Train}}  & \multicolumn{1}{c|}{\textbf{Validation}} & \textbf{Test}   & \multicolumn{1}{c|}{\textbf{Train}}  & \textbf{Test}   & \multicolumn{1}{c|}{\textbf{Train}}  & \multicolumn{1}{c|}{\textbf{Validaiton}} & \textbf{Test}   \\ \hline
\textbf{GPT4-Context Original}   & 0.233           & \multicolumn{1}{c|}{0.6788}          & \multicolumn{1}{c|}{0.7248}              & 0.675           & \multicolumn{1}{c|}{0.5489}          & 0.8351          & \multicolumn{1}{c|}{0.5053}          & \multicolumn{1}{c|}{0.5064}              & 0.5118          \\ \hline
\textbf{GPT4-context-modified}   & \textbf{0.2945} & \multicolumn{1}{c|}{0.6765}          & \multicolumn{1}{c|}{\textbf{0.7407}}     & 0.6749          & \multicolumn{1}{c|}{0.5363}          & \textbf{0.8474} & \multicolumn{1}{c|}{\textbf{0.5767}} & \multicolumn{1}{c|}{\textbf{0.5689}}     & \textbf{0.5674} \\ \hline
\textbf{}                        & \textbf{}       & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\textbf{}}           &                 & \multicolumn{1}{c|}{\textbf{}}       & \textbf{}       & \multicolumn{1}{c|}{\textbf{}}       & \multicolumn{1}{c|}{\textbf{}}           & \textbf{}       \\ \hline
\textbf{GPT3.5-context-original} & 0.2121          & \multicolumn{1}{c|}{0.583}           & \multicolumn{1}{c|}{0.6112}              & 0.5765          & \multicolumn{1}{c|}{0.5383}          & 0.8147          & \multicolumn{1}{c|}{0.4076}          & \multicolumn{1}{c|}{0.3828}              & 0.4197          \\ \hline
\textbf{GPT3.5-context-modified} & \textbf{0.3014} & \multicolumn{1}{c|}{\textbf{0.8021}} & \multicolumn{1}{c|}{\textbf{0.8626}}     & \textbf{0.7902} & \multicolumn{1}{c|}{\textbf{0.543}}  & \textbf{0.8514} & \multicolumn{1}{c|}{\textbf{0.5879}} & \multicolumn{1}{c|}{\textbf{0.5925}}     & \textbf{0.6109} \\ \hline
\textbf{}                        &                 & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                    &                 & \multicolumn{1}{c|}{}                &                 & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                    &                 \\ \hline
\textbf{GPT4-random-original}    & 0.2547          & \multicolumn{1}{c|}{0.7096}          & \multicolumn{1}{c|}{0.7555}              & 0.7068          & \multicolumn{1}{c|}{0.5695}          & 0.8204          & \multicolumn{1}{c|}{0.5719}          & \multicolumn{1}{c|}{0.5775}              & 0.578           \\ \hline
\textbf{GPT4-random-modified}    & \textbf{0.3059} & \multicolumn{1}{c|}{\textbf{0.7421}} & \multicolumn{1}{c|}{\textbf{0.8129}}     & \textbf{0.7357} & \multicolumn{1}{c|}{\textbf{0.5587}} & \textbf{0.8538} & \multicolumn{1}{c|}{0.571}           & \multicolumn{1}{c|}{0.5791}              & 0.5732          \\ \hline
\textbf{GPT4-mixed-original}     & 0.2594          & \multicolumn{1}{c|}{\textbf{0.7289}} & \multicolumn{1}{c|}{\textbf{0.7793}}     & \textbf{0.7233} & \multicolumn{1}{c|}{0.5655}          & \textbf{0.837}  & \multicolumn{1}{c|}{0.5576}          & \multicolumn{1}{c|}{0.5486}              & 0.5579          \\ \hline
\textbf{GPT4-mixed-modified}     & \textbf{0.2979} & \multicolumn{1}{c|}{0.6971}          & \multicolumn{1}{c|}{0.7597}              & 0.6931          & \multicolumn{1}{c|}{\textbf{0.5818}} & 0.8251          & \multicolumn{1}{c|}{\textbf{0.5859}} & \multicolumn{1}{c|}{\textbf{0.5882}}     & \textbf{0.6035} \\ \hline
                                 &                 & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                    &                 & \multicolumn{1}{c|}{}                &                 & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                    &                 \\ \hline
\textbf{GPT3.5-random-original}  & 0.2511          & \multicolumn{1}{c|}{0.6693}          & \multicolumn{1}{c|}{0.7143}              & 0.6705          & \multicolumn{1}{c|}{0.5704}          & 0.8273          & \multicolumn{1}{c|}{0.5646}          & \multicolumn{1}{c|}{0.5556}              & 0.5545          \\ \hline
\textbf{GPT3.5-random-modified}  & \textbf{0.3408} & \multicolumn{1}{c|}{0.6847}          & \multicolumn{1}{c|}{0.7408}              & 0.6802          & \multicolumn{1}{c|}{\textbf{0.5779}} & \textbf{0.8506} & \multicolumn{1}{c|}{0.6161}          & \multicolumn{1}{c|}{\textbf{0.6251}}     & \textbf{0.6201} \\ \hline
\textbf{GPT3.5-mixed-original}   & 0.272           & \multicolumn{1}{c|}{0.6834}          & \multicolumn{1}{c|}{0.7345}              & 0.6827          & \multicolumn{1}{c|}{0.5659}          & 0.831           & \multicolumn{1}{c|}{0.5628}          & \multicolumn{1}{c|}{0.5561}              & 0.5593          \\ \hline
\textbf{GPT3.5-mixed-modified}   & 0.2734          & \multicolumn{1}{c|}{\textbf{0.754}}  & \multicolumn{1}{c|}{\textbf{0.8161}}     & \textbf{0.7456} & \multicolumn{1}{c|}{\textbf{0.585}}  & \textbf{0.8401} & \multicolumn{1}{c|}{\textbf{0.6202}} & \multicolumn{1}{c|}{\textbf{0.6219}}     & \textbf{0.6188} \\ \hline
\end{tabular}
\end{table*}

==> Tables/sent_dataset.tex <==

\begin{table}[]
\begin{tabular}{|c|ccc|cc|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{3}{c|}{Sem Eval 2017}                                  & \multicolumn{2}{c|}{Stanford Sentiment Analsysis} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{Train} & \multicolumn{1}{c|}{Validation} & Test & \multicolumn{1}{c|}{Train}      & Validation      \\ \hline
Positive               & \multicolumn{1}{c|}{17489} & \multicolumn{1}{c|}{819}        & 2375 & \multicolumn{1}{c|}{37569}      & 444             \\ \hline
Negative               & \multicolumn{1}{c|}{7093}  & \multicolumn{1}{c|}{312}        & 3972 & \multicolumn{1}{c|}{29780}      & 428             \\ \hline
Neutral                & \multicolumn{1}{c|}{20673} & \multicolumn{1}{c|}{869}        & 5937 & \multicolumn{1}{c|}{-}          & -               \\ \hline
\end{tabular}
\end{table}


==> ablation.tex <==
% As previously stated, we hypothesize that the generated context would better help align the emotional content of the sentence to the assigned emotional label. The presented results confidently verify this assumption. However, our framework of adding context should consider that the context is dependent on the input sentence. Hence, we provide an ablation study, in which we train a BERT model as described in Section [Experiments] with only containing the generated context sentence and excluding the original sentence from Go Emotions. The zero-shot results are seen in Figure~[]. These results validate our hypothesis that the context is dependent on the input sentence and would not make complete sentences without the base sentence.

